Understanding Social Structures from Contemporary Literary Fiction using Character Interaction Graph -- Half Century Chronology of Influential Bengali Writers

Social structures and real-world incidents often influence contemporary literary fiction. Existing research in literary fiction analysis explains these real-world phenomena through the manual critical analysis of stories. Conventional Natural Language Processing (NLP) methodologies, including sentiment analysis, narrative summarization, and topic modeling, have demonstrated substantial efficacy in analyzing and identifying similarities within fictional works. However, the intricate dynamics of character interactions within fiction necessitate a more nuanced approach that incorporates visualization techniques. Character interaction graphs (or networks) emerge as a highly suitable means for visualization and information retrieval from the realm of fiction. Therefore, we leverage character interaction graphs with NLP-derived features to explore a diverse spectrum of societal inquiries about contemporary culture's impact on the landscape of literary fiction. Our study involves constructing character interaction graphs from fiction, extracting relevant graph features, and exploiting these features to resolve various real-life queries. Experimental evaluation of influential Bengali fiction over half a century demonstrates that character interaction graphs can be highly effective in specific assessments and information retrieval from literary fiction. Our data and codebase are available at https://cutt.ly/fbMgGEM

==> backup.tex <==
\begin{table*}[h]
\centering
\begin{tabular}{l|l}
\hline
Year      & Event     \\                                    \hline                                                                                                                                                                        
1872      & The Brahma Marriage Act passed lifting ban on widow remarriage                                                                                                                                                                               \\
1882      & Women enter university                                                                                                                                                                                                                       \\
1885      & Bengal Tenancy Act                                                                                                                                                                                                                           \\
1905      & First Partition of Bengal; spearheading the ‘Quit India’ Movement                                                                                                                                                                            \\
% 1906      & \begin{tabular}[c]{@{}l@{}}Bengali Brahma start the Society for the Improvement of Backward Classes,  which is the \\ earliest pioneering movement in India dedicated to ameliorating the conditions of Hindu \\  untouchables.\end{tabular} \\
1911      & Annulment of Bengal Partition                                                                                                                                                                                                                \\
1912      & Imperial capital shifted from Calcutta to Delhi                                                                                                                                                                                              \\
1914-1918 & Fall in jute prices affects the Bengal economy and  WW-I  effect                                                                                                                                                                                      \\
1917      & Influence of Bolshevism in Bengal intelligentsia                                                                                                                                                                                             \\
1919      & Jallianwala Bagh massacre                                                                                                                                                                                                                    \\
1920      & Non-cooperation movement against colonial rulers led by Gandhi; and civil   disobedience                                                                                    \\
1930      & Salt march movement by Gandhi  \\
\hline
\end{tabular}
\caption{Political and social events in contemporary time of late nineteenth and early twentieth century }
\label{tab-events}
\end{table*}

==> genre_protagonist_table.tex <==
%\setlength{\tabcolsep}{1pt}

% Please add the following required packages to your document preamble:
% \usepackage[table,xcdraw]{xcolor}
% If you use beamer only pass "xcolor=table" option, i.e. \documentclass[xcolor=table]{beamer}
\begin{table}[t]
\caption{Year-wise Story, Genre and Protagonist Information for All Authors}
\label{tab-protagonist}
\setlength{\tabcolsep}{2pt}
\begin{tabular}{lll|lll|lll}
\toprule
\multicolumn{3}{|c|}{Bankim Chandra}                                                                                                                                        & \multicolumn{3}{c|}{Rabindranath Tagore}                                                                                                                                    & \multicolumn{3}{c|}{Sarat Chandra Chattopadhyay}                                                                                                                      \\ \toprule
Story name                                                          & Genre                                                          & P                                    & Story name                                                           & Genre                                                         & P                                    & Story name                                                       & Genre                                                       & P                                    \\ 
\midrule
\begin{tabular}[c]{@{}l@{}}Durgeshnan\\ dini(1865)\end{tabular}     & \begin{tabular}[c]{@{}l@{}}Historical \\ Romantic\end{tabular} & {\color[HTML]{00009B} \textbf{F-A2}} & \begin{tabular}[c]{@{}l@{}}Bou Thakuran\\ ir Haat(1883)\end{tabular} & Historical                                                    & {\color[HTML]{00009B} \textbf{F-A2}} & \begin{tabular}[c]{@{}l@{}}Borodidi\\ (1907)\end{tabular}        & Social                                                      & {\color[HTML]{9A0000} \textbf{M-A2}} \\ \hline
\begin{tabular}[c]{@{}l@{}}Kapalakun\\ dala(1866)\end{tabular}      & {\color[HTML]{F56B00} Romantic}                                & {\color[HTML]{00009B} \textbf{F-A2}} & \begin{tabular}[c]{@{}l@{}}Chokher Bali\\ (1901)\end{tabular}        & \begin{tabular}[c]{@{}l@{}}Social,\\ Romantic\end{tabular}    & {\color[HTML]{00009B} \textbf{F-A2}} & \begin{tabular}[c]{@{}l@{}}Devdas\\ (1914)\end{tabular}          & {\color[HTML]{F56B00} Romantic}                             & {\color[HTML]{9A0000} \textbf{M-A2}} \\ \hline
\begin{tabular}[c]{@{}l@{}}Mrinalini\\ (1869)\end{tabular}          & \begin{tabular}[c]{@{}l@{}}Historical \\ Romantic\end{tabular} & {\color[HTML]{00009B} \textbf{F-A2}} & \begin{tabular}[c]{@{}l@{}}Noukadubi\\ (1906)\end{tabular}           & \begin{tabular}[c]{@{}l@{}}Social, \\ Romantic\end{tabular}   & {\color[HTML]{9A0000} \textbf{M-A2}} & \begin{tabular}[c]{@{}l@{}}Panditama\\  sai(1914)\end{tabular}    & \begin{tabular}[c]{@{}l@{}}Social,\\ Romantic\end{tabular}  & {\color[HTML]{9A0000} \textbf{M-A2}} \\ \hline
Indira(1873)                                                        & Social                                                         & {\color[HTML]{00009B} \textbf{F-A2}} & Gora(1909)                                                           & \begin{tabular}[c]{@{}l@{}}Political,\\ Romantic\end{tabular} & {\color[HTML]{9A0000} \textbf{M-A2}} & \begin{tabular}[c]{@{}l@{}}Pallisamaj\\ (1916)\end{tabular}      & Social                                                      & {\color[HTML]{9A0000} \textbf{M-A2}} \\  \hline
\begin{tabular}[c]{@{}l@{}}Bisabrksa\\ (1873)\end{tabular}          & Social                                                         & {\color[HTML]{963400} \textbf{M-A2}} & \begin{tabular}[c]{@{}l@{}}Ghare Baire\\ (1916)\end{tabular}         & {\color[HTML]{32CB00} Political}                              & {\color[HTML]{9A0000} \textbf{M-A2}} & \begin{tabular}[c]{@{}l@{}}Chandranath\\ (1916)\end{tabular}     & \begin{tabular}[c]{@{}l@{}}Social, \\ Romantic\end{tabular} & {\color[HTML]{00009B} \textbf{F-A2}} \\  \hline
\begin{tabular}[c]{@{}l@{}}Yugalangu\\ riya(1874)\end{tabular}      & {\color[HTML]{F56B00} Romantic}                                & {\color[HTML]{00009B} \textbf{F-A1}} & \begin{tabular}[c]{@{}l@{}}Chaturanga\\ (1916)\end{tabular}          & Social                                                        & {\color[HTML]{9A0000} \textbf{M-A2}} & \begin{tabular}[c]{@{}l@{}}Baikunther \\ Will(1916)\end{tabular} & Social                                                      & {\color[HTML]{9A0000} \textbf{M-A2}} \\  \hline
\begin{tabular}[c]{@{}l@{}}Radharani\\ (1876)\end{tabular}          & \begin{tabular}[c]{@{}l@{}}Social, \\ Romantic\end{tabular}    & {\color[HTML]{00009B} \textbf{F-A1}} & \begin{tabular}[c]{@{}l@{}}Shesher\\ Kabita (1929)\end{tabular}      & {\color[HTML]{F56B00} Romantic}                               & {\color[HTML]{9A0000} \textbf{M-A2}} & \begin{tabular}[c]{@{}l@{}}Parinita\\ (1916)\end{tabular}        & {\color[HTML]{F56B00} Romantic}                             & {\color[HTML]{00009B} \textbf{F-A1}} \\  \hline
\begin{tabular}[c]{@{}l@{}}Chandra\\ sekhar(1877)\end{tabular}      & Social                                                         & {\color[HTML]{9A0000} \textbf{M-A2}} & Jogajog(1929)                                                        & Social                                                        & {\color[HTML]{00009B} \textbf{F-A2}} & \begin{tabular}[c]{@{}l@{}}Araksaniya\\ (1916)\end{tabular}      & Social                                                      & {\color[HTML]{00009B} \textbf{F-A3}} \\  \hline
Rajani(1877)                                                        & {\color[HTML]{F56B00} Romantic}                                & {\color[HTML]{00009B} \textbf{F-A2}} & \begin{tabular}[c]{@{}l@{}}Dui bon\\ (1933)\end{tabular}             & Social                                                        & {\color[HTML]{00009B} \textbf{F-A2}} & \begin{tabular}[c]{@{}l@{}}Niskriti\\ (1917)\end{tabular}        & Social                                                      & {\color[HTML]{00009B} \textbf{F-A2}} \\ \hline
\begin{tabular}[c]{@{}l@{}}Krishnakanter \\ Will(1878)\end{tabular} & Social                                                         & {\color[HTML]{9A0000} \textbf{M-A3}} & \begin{tabular}[c]{@{}l@{}}Malancha\\ (1934)\end{tabular}            & Social                                                        & {\color[HTML]{00009B} \textbf{F-A2}} & \begin{tabular}[c]{@{}l@{}}Charitrohin\\ (1917)\end{tabular}     & Social                                                      & {\color[HTML]{9A0000} \textbf{M-A2}} \\  \hline
\begin{tabular}[c]{@{}l@{}}Anandamath\\ (1882)\end{tabular}         & {\color[HTML]{009901} Political}                               & {\color[HTML]{9A0000} \textbf{M-A2}} & \begin{tabular}[c]{@{}l@{}}Char Odhhay\\ (1934)\end{tabular}         & {\color[HTML]{009901} Political}                              & {\color[HTML]{00009B} \textbf{F-A2}} & Datta(1918)                                                      & \begin{tabular}[c]{@{}l@{}}Social, \\ Romantic\end{tabular} & {\color[HTML]{00009B} \textbf{F-A2}} \\  \hline
\begin{tabular}[c]{@{}l@{}}Devi Chaudhu\\ rani(1884)\end{tabular}   & \begin{tabular}[c]{@{}l@{}}Historical\\ Romantic\end{tabular}  & {\color[HTML]{00009B} \textbf{F-A2}} &                                                                      &                                                               &                                      & \begin{tabular}[c]{@{}l@{}}Grihodaho\\ (1920)\end{tabular}       & \begin{tabular}[c]{@{}l@{}}Social, \\ Romantic\end{tabular} & {\color[HTML]{00009B} \textbf{F-A2}} \\ \cline{7-9}
                                                                    &                                                                &                                      &                                                                      &                                                               &                                      & \begin{tabular}[c]{@{}l@{}}Dena Paona\\ (1923)\end{tabular}      & \begin{tabular}[c]{@{}l@{}}Social, \\ Romantic\end{tabular} & {\color[HTML]{00009B} \textbf{F-A2}} \\ \cline{7-9}
                                                                    &                                                                &                                      &                                                                      &                                                               &                                      & \begin{tabular}[c]{@{}l@{}}Nababidha\\ (1924)\end{tabular}       & \begin{tabular}[c]{@{}l@{}}Social, \\ Romantic\end{tabular} & {\color[HTML]{9A0000} \textbf{M-A2}} \\ \cline{7-9}
                                                                    &                                                                &                                      &                                                                      &                                                               &                                      & \begin{tabular}[c]{@{}l@{}}Pather Dabi\\ (1926)\end{tabular}     & {\color[HTML]{009901} Political}                            & {\color[HTML]{9A0000} \textbf{M-A2}} \\ \cline{7-9}
                                                                    &                                                                &                                      &                                                                      &                                                               &                                      & \begin{tabular}[c]{@{}l@{}}Shesprasna\\ (1931)\end{tabular}      & Social                                                      & {\color[HTML]{00009B} \textbf{F-A2}} \\
                                                                    \bottomrule
\end{tabular}
\end{table}
